A LoRa-based Energy-efficient Sensing System for Urban Data Collection

Nowadays, cities provide much more than shopping opportunities or working spaces. Individual locations such as parks and squares are used as meeting points and local recreation areas by many people. To ensure that they remain attractive in the future, the design of such squares must be regularly adapted to the needs of the public. These utilization trends can be derived using public data collection. The more diverse and rich the data sets are, the easier it is to optimize public space design through data analysis. Traditional data collection methods such as questionnaires, observations, or videos are either labor intensive or cannot guarantee to preserve the individual's privacy. This work presents a privacy-preserving, low-power, and low-cost smart sensing system that is capable of anonymously collecting data about public space utilization by analyzing the occupancy distribution of public seating. To support future urban planning the sensor nodes are capable of monitoring environmental noise, chair utilization, and their position, temperature, and humidity and provide them over a city-wide Long Range Wide Area Network (LoRaWAN). The final sensing system's robust operation is proven in a trial run at two public squares in a city with 16 sensor nodes over a duration of two months. By consuming 33.65 mWh per day with all subsystems enabled, including sitting detection based on a continuous acceleration measurement operating on a robust and simple threshold algorithm, the custom-designed sensor node achieves continuous monitoring during the 2-month trial run. The evaluation of the experimental results clearly shows how the two locations are used, which confirms the practicability of the proposed solution. All data collected during the field trial is publicly available as open data.

==> src/02_RelatedWork.tex <==
%-------------------------------------------------------------------------------------------------------------------
% Related Work
%-------------------------------------------------------------------------------------------------------------------
\section{Related Work}\label{sec:relatedwork}
% maybe more introduction...
% The concept of smart cities conflates several service domains of today's cities and aims to improve their efficiency in a multitude
% of possible ways \cite{yang_smart_city_development_2021}.
%Managing natural and energy resources at city-level \cite{carli_smart_city_energy_management_2017} down to individual smart buildings %\cite{metallidou_smart_building_efficiency_2020} allows to use the existing energy sensibly and thus reducing the gap between energy
%consumption and demand \cite{mulero_ressource_planning_2020}.
%In the transportation and mobility sector, intelligent control algorithms can use dynamic data of several sensors to improve the street's 
%utilization and reduce traffic congestion \cite{kong_bus_profiling_2020}.
%To facilitate infrastructure maintenance, smart sensors can help to detect if and when service is needed, for example waste management \cite{khan_smart_waste_management_2021}. \\

Urban computing in smart cities relies on big data collection and analysis. 
Many locations are suitable for gathering data, however, the location and the type of data may depend on the topic of interest.
Focusing on the improvement of public spaces, simple approaches like pedestrian counting \cite{de_ruyter_automatic_2010} can already indicate how often a certain location is visited. Many experimental as well as commercial sensing systems already allow for measuring pedestrian utilization at fixed positions in a city \cite{akhter_iot_2019, akhter_design_2019}.
In addition to people counting, data originating from social media or cell phones can be utilized as a means to assess the usage of public spaces \cite{ciuccarelli_visualizing_2014}. It has the benefit of encompassing the entire metropolis rather than being restricted to a single area.
While the latter two approaches provide reliable insights into the usage of city spaces such as shops, stairways, and elevators over time, the usage of public infrastructure like benches or chairs, but also shaded places cannot be precisely measured. \\
Installing local sensor nodes for specific sensing tasks could complement already existing solutions in specific areas \cite{lau_sensor_fusion_monitoring_2018}. 
For example, by leveraging wireless communication \cite{rashid_applications_2016, carminati_prospects_2019}, only people being present at squares are accounted for,  but not if they use the provided seating, prefer sunny places or shaded ones or prefer loud or quiet environments. 
Questionnaires and local observations can gather those missing measurement values, but they are time-consuming, and labor-intensive, and do not provide constant data over a long period of time. 


%-------------------------------------------------------------------------------------------------------------------
% End Related Work
%-------------------------------------------------------------------------------------------------------------------
